Energy conserving and well-balanced discontinuous Galerkin methods for the Euler-Poisson equations in spherical symmetry

This paper presents high-order Runge-Kutta (RK) discontinuous Galerkin methods for the Euler-Poisson equations in spherical symmetry. The scheme can preserve a general polytropic equilibrium state and achieve total energy conservation up to machine precision with carefully designed spatial and temporal discretizations. To achieve the well-balanced property, the numerical solutions are decomposed into equilibrium and fluctuation components which are treated differently in the source term approximation. One non-trivial challenge encountered in the procedure is the complexity of the equilibrium state, which is governed by the Lane-Emden equation. For total energy conservation, we present second- and third-order RK time discretization, where different source term approximations are introduced in each stage of the RK method to ensure the conservation of total energy. A carefully designed slope limiter for spherical symmetry is also introduced to eliminate oscillations near discontinuities while maintaining the well-balanced and total-energy-conserving properties. Extensive numerical examples -- including a toy model of stellar core-collapse with a phenomenological equation of state that results in core-bounce and shock formation -- are provided to demonstrate the desired properties of the proposed methods, including the well-balanced property, high-order accuracy, shock capturing capability, and total energy conservation.

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

%
%% Packages and macros go here
%\usepackage{amsfonts}
%\usepackage{graphicx,epstopdf}
%\usepackage{mathrsfs}
%\usepackage{bm}
%\usepackage{multirow}
%%\usepackage{cite}
%\usepackage{color}
%\usepackage{hyperref} 
%\hypersetup{colorlinks=false} %
%
%\usepackage{caption, subcaption}%
%\usepackage{array}
%\usepackage{enumitem}   
%
%\usepackage{xparse} % for {{}}
%\usepackage{stmaryrd} % for [[]]

%use by Y. Xu, C.-W. Shu and Q. Zhang, Error estimate of the fourth order Runge-Kutta discontinuous Galerkin methods for linear hyperbolic equations, submitted to SIAM Journal on Numerical Analysis.
\usepackage{geometry}
%\geometry{left=3.15cm,right=3.15cm,top=2.79cm,bottom=2.92cm}
\geometry{left=3.15cm,right=3.15cm,top=2.62cm,bottom=2.75cm}
%
%
%%% Used for creating new theorems, remarks
%\newsiamthm{claim}{Claim}
%\newsiamremark{remark}{Remark}
%\newsiamremark{expl}{Example}
%%\newsiamthm{proposition}{Proposition}
%%\newsiamremark{hypothesis}{Hypothesis}
%%\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\numberwithin{theorem}{section}
%\newcounter{example}

%\setlength{\textwidth}{5.26in} 
%\setlength{\textheight}{8.48in}
%\hoffset=-0.02truein 
%\voffset=-0.09truein

%\renewcommand\baselinestretch{0.988}
\allowdisplaybreaks

\usepackage{amsopn}
\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{makecell}
\usepackage{ulem}
%%%%%%
%%	Personal head with min imum of usefull packages,
%%	ntheorem environment and shortenings
\usepackage{verbatim}
\usepackage{fancyhdr}
\usepackage{verbatim}
\usepackage{fancyhdr}
\usepackage{indentfirst}
\usepackage[ansinew]{inputenc}
\usepackage{booktabs}
\usepackage{amssymb}
\usepackage{amsmath,amssymb,graphicx}
%\usepackage{amsthm}
\usepackage{subfigure}
\usepackage{color}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{listings}
\usepackage{array}
\usepackage{booktabs}
%\usepackage{titlesec}
\usepackage{float}
\usepackage{appendix}
\usepackage{tikz}
\usepackage{caption}
%\usepackage{caption, subcaption}%
\theoremseparator{.}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{example}{Example}[section]
\newtheorem{remark}[theorem]{Remark}
\numberwithin{theorem}{section}
\numberwithin{equation}{section}
\numberwithin{table}{section}
\numberwithin{figure}{section}
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\renewcommand{\thetable}{\arabic{section}.\arabic{table}}
\renewcommand{\thefigure}{\arabic{section}.\arabic{figure}}
%\usepackage[colorlinks,
%linkcolor=blue,
%anchorcolor=blue,
%citecolor=blue]{hyperref}
%\theorembodyfont{\upshape}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{proof}{Proof}
\graphicspath{{./figures/}}  % to set figure path.
\newcommand{\YX}[1]{{\color{red} [#1]}}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}


% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Energy conserving and well-balanced discontinuous Galerkin methods for the Euler-Poisson equations in spherical coordinate} 
\newcommand{\TheAuthors}{Weijie Zhang, Eirik Endeve and Yulong Xing}

% Sets running headers as well as PDF title and authors
%\headers{}
%{xxx and xxx}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{{\TheTitle}} %\thanks{Submitted to the editors on \today.}
\title{{\TheTitle}\thanks{Submitted to the journal. \funding{This work was carried out when W. Zhang was visiting Department of Mathematics, The Ohio State University under the support of the China Scholarship Council (CSC NO. 201906340196). The work of E. Endeve is partially supported by \YX{xxx}. The work of Y. Xing is partially supported by the NSF grant DMS-1753581.}}}

% Authors: full names plus addresses.
\author{	Weijie Zhang\thanks{\YX{xxx} University of Kansas, (\email{xxx}).}
		\and Eirik Endeve\thanks{\YX{xxx} Oak Ridge National Laboratory, (\email{xxx}).} 
		\and Yulong Xing\thanks{Department of Mathematics, The Ohio State University,
		Columbus, OH 43210, USA (\email{xing.205@osu.edu}).}}




%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

